On The Reachability Problem for Recursive Hybrid Automata with One and Two Players

Motivated by the success of bounded model checking framework for finite state machines, Ouaknine and Worrell proposed a time-bounded theory of real-time verification by claiming that restriction to bounded-time recovers decidability for several key decision problem related to real-time verification. In support of this theory, the list of undecidable problems recently shown decidable under time-bounded restriction is rather impressive: language inclusion for timed automata, emptiness problem for alternating timed automata, and emptiness problem for rectangular hybrid automata. The objective of our study was to recover decidability for general recursive timed automata---and perhaps for recursive hybrid automata---under time-bounded restriction in order to provide an appealing verification framework for powerful modeling environments such as Stateflow/Simulink. Unfortunately, however, we answer this question in negative by showing that time-bounded reachability problem stays undecidable for recursive timed automata with five or more clocks. While the bad news continues even when one considers well-behaved subclasses of recursive hybrid automata, we recover decidability by considering recursive hybrid automata with bounded context using a pass-by-reference mechanism, or by restricting the number of variables to two, with rates in $\{0,1\}$.

==> dec-ref-full-app.tex <==
We adapt the contraction operator $cnt$ of \cite{BG13} and make it {\it context-sensitive}.  This operator
respects the context of the RHA configurations. Given a run $\rho$ in RHA with call-by-reference 
only mechanism, we split into type-3 runs exactly as done for hybrid automata \cite{BG13}. While applying contraction, 
we identify repetition of configurations by matching not just the location but the (context, location) pair in the configurations. The context matching ensures that we do not alter the sequence of recursive calls made in the contracted run, thus maintaining validity w.r.t recursion. The second occurence is then deleted and the time delays are added to the first occurence of the loop. Let us denote the (context, location) pair to be used for matching as $cl = (\sseq{\kappa},q)$.

\begin{lemma}
 \label{lem:cnt-len-type3}
 Given a type-3 run $\rho$ in the bounded context RHA $H$, $|cnt^*(\rho)| \leq (\alpha .|Q| . (2.cmax+1)^{|\variables|})^2 +1$, where 
  $\alpha=\sum\limits_{i=1}^K n^i$, $K$ is the bound on the context length, and $n$ is the number of boxes in $H$.
\end{lemma}
\begin{proof}
 Contraction of \cite{BG13}, matches the locations in a type-3 run. Thus the size of a contracted type-3 run is $|Loc|^2+1$ (Lemma 7 of \cite{BG13}) where $Loc$ is the set of locations in the region hybrid automata. However, we match (context,location) pairs in our context-sensitive contraction. 

Suppose $\rho$ is a type-3 run. Let $\rho' = cnt^*(\rho)$ have $M$ unique context, location pairs. 
Highlighting the first occurrences of these $M$ unique pairs and ignoring the valuations, we have in $\rho'$, 
$\underline{(\sseq{\kappa_1},q_1)} w_1 \underline{(\sseq{\kappa_2},q_2)} w_2 \dots  \underline{(\sseq{\kappa_{M-1}},q_{M-1})} w_{M-1} \underline{(\sseq{\kappa_M},q_M)} w_M$
where $w_i$ are strings over (context,location) pairs, which does not have any first occurrence of a 
(context,location) pair.  Clearly,  there are $M$ first occurences of (context, location) 
pairs $((\sseq{\kappa_i},q_i)$ for $1 \leq i \leq M$. Let a {\it portion} be a part of $\rho'$ between two such first occurences $(\sseq{\kappa_{i-1}},q_{i-1})$ and 
$(\sseq{\kappa_i},q_i)$, $2 \leq i \leq M+1$. 
  In a portion, contraction cant be applied anymore. If could be, then $cnt^*(\rho)$ is not a fixpoint.
    There could be a $cl$ pair such that 
    its first occurrence is at index $i$, and second occurrence is at index $j$, $i< j$; that is, 
    $cl_i=(\sseq{\kappa_i},q_i)=(\sseq{\kappa_j},q_j)=cl_j$, and the index $j$ is part of 
    a later portion ($cl_i$ is thus underlined, but $cl_j$ is not). We cannot contract the pairs at indices $i,j$, since 
         {\it all pairs} between $cl_i$ and $cl_j$ would not occur prior to $cl_i$ (if they occur, then 
         $\rho' \neq cnt^*(\rho))$. 
                  Thus the number of unique pairs in a portion could be more than 1 and can be atmost $M$. Thus the maximum length of $\rho' \leq M^2+1$. 

There are atmost $\alpha = \sum\limits_{i=1}^K n^i$ different contexts of size atmost $K$ with any sequence of the $n$ boxes including a box being called more than once. We know that $M$ is the number of unique (context, location) pairs. 
Clearly, $M \leq \alpha . |Q| . (2.cmax+1)^{|\variables|} $, where $Q=\bigcup_{i=1}^nQ_i$ is the union of the set of vertices $Q_i$ of all the $n$ components of the RHA, $|Q|.(2.cmax+1)^{|\variables|}$ is the number of vertices in the region RHA and $K$ is the context bound. Thus, the length of a type-3 contracted run is $(\alpha . |Q|. (2.cmax+1)^{|\variables|} )^2+1$. Thus proved.
\end{proof}

Let us illustrate with an example why a contracted type-3 run $|cnt^*(\rho)|$ could be of length $>\alpha .|Q|. (2.cmax+1)^{|\variables|}$. Let $CL$ be a set of unique (context, location) pairs ($|CL| \leq \alpha . |Q|. (2.cmax+1)^{|\variables|}$). Assume $CL = \set{a,b,c,d,e,f}$. Let us abuse notation of a run for a short while and depict it to be only a sequence of pairs ignoring the valuations. Now let $cnt^*(\rho) = \rho'= \underline{a} \rightarrow \underline{b} \rightarrow \underline{c}\rightarrow \underline{d}\rightarrow a\rightarrow \underline{e} \rightarrow b\rightarrow \underline{f}$. Here the portions are 
$\epsilon$ (between $a$ and $b$, between $b$ and $c$, and between $c$ and $d$) and 
$a$ (between $d$ and $e$) and $b$ (between $e$ and $f$). 
%$a$, $b$, $c$, $d\rightarrow a$, $e\rightarrow b$ and $f$.
 Note that each of these portions themselves can not be contracted any further. Additionally although there are two occurences of $a$ (position 0 and 4) itself, the pairs between the first and second occurence of $a$ (these pairs are $b,c,d$) do not appear prior to $a$ at position 0. Thus contraction can not be applied to $\rho'$. Thus $|cnt^*(\rho)|$ could be $>\alpha . |Q|.(2.cmax+1)^{|\variables|}$. However, each portion itself could be atmost $\alpha . |Q|.(2.cmax+1)^{|\variables|}$ (number of unique pairs). Thus $|cnt^*(\rho)| \leq (\alpha . |Q|.(2.cmax+1)^{|\variables|})^2+1$

\begin{lemma}
 \label{lem:cnt-len}
 Given a run $\rho$ in the bounded context RHA $H$, $|cnt^*(\rho)| \leq 24 (T.rmax +1 ) |\variables|^2  (\alpha |Q|)^2. (2 .cmax + 1)^{2 |\variables|}$.
\end{lemma}
\begin{proof}
Recall the splitting of a given run prior to contraction detailed in Section \ref{sec:decidability}. The given run $\rho$ (type-0) yeilds $(T.rmax+1)$ type-1 runs each of which is further split into $(3.|\variables|)$ type-2 runs. Each type-2 run is split into $2.|\variables|+1$ type-3 runs. Each contracted type-3 run is atmost $(\alpha. |Q|.(2.cmax+1)^{|\variables|})^2+1$ long (Lemma \ref{lem:cnt-len-type3} above). Thus each length of contracted type-2 run is

$\begin{array}{l}
\leq [2.|\variables|+1].[(\alpha. |Q|.(2.cmax+1)^{|\variables|})^2+1] \\
\leq 2 . (|\variables|+1). ((\alpha. |Q|.(2.cmax+1)^{|\variables|})^2+1) \\
\leq 2 . (2.|\variables|). (2.(\alpha. |Q|.(2.cmax+1)^{|\variables|})^2)  \\
= 8 . |\variables| .(\alpha. |Q|.(2.cmax+1)^{|\variables|})^2 \\
\end{array}
$
\newline
Thus the length of $cnt^*(\rho) \leq [(T.rmax+1) . (3.|\variables|)]~.~[8 . |\variables| .(\alpha. |Q|.(2.cmax+1)^{|\variables|})^2] = 24 (T.rmax+1).|\variables|^2.(\alpha. |Q|)^2.(2.cmax+1)^{2.|\variables|}$. Thus proved. 

%  Splitting of $\rho$ into type-1, type-2 and type-3 runs, yields $24 (T . rmax +1 )  |\variables| ^2  (2 . cmax + 1)^{2 |\variables|}$ type-3 runs \cite{BG13}. From Lemma \ref{lem:cnt-len-type3} above, the length of a contracted type-3 run is atmost $(\alpha|Q|)^2+1$. Thus proved.
\end{proof}


\begin{lemma}
 \label{lem:cnt-valid}
 Given a run $\rho$ in the bounded context RHA $H$, $cnt^*(\rho)$ is a valid run in $H$. 
\end{lemma}
\begin{proof}
To prove that the contracted run $\rho'$ is valid in the given bounded context RHA $H$, we need to ensure two conditions : 
\begin{itemize}
 \item the constraints appearing along the transitions of $\rho'$ are still satisfied and 
 \item the sequence of boxes (and mapping of call, return, entry, exit vertices) is valid w.r.t recursive calls in the given RHA. This means call port and appropriate entry node should be consecutive in the contracted run, exit node-return ports are matched and the contexts in configurations of $\rho'$ should be valid successors of the preceeding contexts.   
\end{itemize}
  
The first condition is satisfied as we consider a variant of RHA where all the variables are always 
passed by reference. Thus the context has no valuations but only a sequence of boxes. The constraints 
are guaranteed to be satisfied as the run is same as a hybrid automata run if the context is ignored. 
Thus the precautions (in carefully splitting from type-0 to type-3 runs) taken in \cite{BG13} for hybrid automata suffice with regards to constraints. 
 
The second condition is satisfied due to context-sensitive contraction where in the context is also matched 
in the loop detection. Due to this, a context in the contracted run will be a valid successor of the preceeding 
 context. We shall prove by contradiction that there exists no invalid pair of consecutive configurations in the contracted run $\rho'$. There are several ways in which a pair of configurations can be invalid predecessor/successor w.r.t recursion: 
 \begin{itemize}
  \item the call port and entry node are mismatched (either of them is missing or matched to another box's entry node)
  \item the return node and exit port are mismatched
  \item the consecutive contexts are incorrect/invalid 
 (the sequences of boxes in the two contexts are such that it is not possible in the RHA semantics to get one sequence from another via a valid RHA move.) 
 \end{itemize}

 Suppose there exists a pair of consecutive configurations 
 in $\rho'$ which are invalid w.r.t recursive call. For ease of explanation, lets call the successor of a configuration $c$ in $\rho$ as $succ(c)$ and its predecessor as $pred(c)$. Abusing notation, we henceforth consider the context $\kappa \in B^*$ as all variables are always passed by reference and hence need not be stored in the context.
 
Let us assume that the contracted run has a pair of consecutive configurations $c' \stackrel{t,e}{\rightarrow} d'$ which are invalid as the call port configuration $c'$ is not succeeded by the appropriate entry node configuration in the contracted run i.e; $c' = (\sseq{\kappa},(b,en),\nu')$ and $d' \neq (\sseq{\kappa,b},en,\nu')$. Consider configurations $c = (\sseq{\kappa},(b,en),\nu)$ and $succ(c)= (\sseq{\kappa,b},en,\nu)$ in the given run $\rho$ such that $c'$ corresponds to $c$. As $d' \neq (\sseq{\kappa,b},en,\nu')$, the configuration $succ(c)$ was deleted during contraction. Thus it must be the case that in $\rho$, $c$ was at position $i$ while the repeated (context,location) pairs were from position $i+1$ to $j$ and $d$ (corresponding to $d'$ in $\rho'$) was at position $j+1$. But, the configuration at $i+1$ is $succ(c)$ and this was matched with a configuration, say $e$ occuring prior to $c$ in $\rho$ : recall the contraction operator deletes 
repeating occurrences of (location, context) pairs; to delete $succ(c)$ at position $i+1$, 
we have to match the  (location, context) pair of $succ(c)$ at position $i+1$ with that of some 
$e$, occurring at a position $m < i$.  
   Due to the semantics of RHA, $pred(e)$ has (context, location) pair $(\sseq{\kappa},(b,en))$ which is the same as $c$. Thus even $c$ would be matched to $pred(e)$ and deleted. This contradicts our assumption that $c'$ (equivalent of $c$) exists in $\rho'$. 

In essence, the call port-entry node configurations always appear consecutive to each other in a given run $\rho$. Thus, matching a call-port configuration to a configuration $c$ will invariably match the corresponding entry-node configuration to the $succ(c)$ which will also be the same entry-node configuration. Similarly, exit-node and corresponding return-port configurations always appear consecutive to each other.

Now, lets consider another pair of invalid consecutive configurations $c_1' \stackrel{t,e}{\rightarrow} c_2'$ in $\rho'$ such that $c_1' = (\sseq{b_1},q_1,\nu_1')$ and $c_2' = (\sseq{b_1b_2b_3},q_2,\nu_2')$. Clearly, such a sequence is invalid under the RHA semantics (even if $q_1$ is a call port). During context-sensitive contraction, we match the (context,location) pairs and do not alter the contexts. Now consider two configurations $c_1$ and $c_2$ in $\rho$ which correspond to $c_1'$ and $c_2'$ respectively. Hence  $c_1 = (\sseq{b_1},q_1,\nu_1)$ and $c_2 = (\sseq{b_1b_2b_3},q_2,\nu_2)$ (valuations would differ in the two paths due to contraction). Obviously $c_2$ is not successor of $c_1$ in $\rho$, as $\rho$ is the given run (hence valid) and hence cant have such a pair of consecutive configurations. For $c_1' \stackrel{t,e}{\rightarrow} c_2'$ in $\rho'$, it must be the case that in $\rho$, $c_1$ is the $i$th configuration and the repeated (context,location) pairs are from $i+1$ to $j$ and $c_2$ is the 
$j+1$ configuration. 
Let $pred(c_2)$ be the predecessor of $c_2$ in $\rho$, i.e; the configuration appearing at position $j$. Contraction deletes the configurations from $i+1$ to $j$ and hence $c_2'$ ends up as successor of $c_1'$. 
However, from the definition of contraction (\cite{BG13}) seen earlier in Section \ref{sec:decidability}, we know that (context, location) pair of $c_1$ is the same as that of $pred(c_2)$ (recall that $(l_i,context_i) = (l_j,context_j)$). Thus context of $pred(c_2)$ is $\sseq{b_1}$ which can not be followed by $\sseq{b_1b_2b_3}$ of $c_2$ in $\rho$. Thus contradicting our assumption that $c_2'$ succeeds $c_1'$ in $\rho'$.

Similar proof by contradiction can be given for any pair of configurations invalid w.r.t recursion.
\end{proof}

\begin{theorem}
 \label{thm:dec-ref}
 Time bounded reachability is decidable for bounded context RHA using only call-by-reference mechanism.
\end{theorem}
\begin{proof}
 Contraction of a given run $\rho$ yields a smaller run $\rho'$ whose length is independent of $\rho$. From Lemma \ref{lem:cnt-len}, we know that $|\rho'| \leq C= 24 (T .rmax +1 )  |\variables| ^2  [(\alpha |Q|)^2+1]  (2 .cmax + 1)^{2  |\variables|}$. Additionally, from Lemma \ref{lem:cnt-valid}, $\rho'$ is a valid run in the RHA. Thus a non-deterministic algorithm (as in the case of Hybrid automata \cite{BG13}) can be used to guess a run of length atmost $C$ and then solve an  LP to check if there are time values and valuations for each step that make such a run feasible. Thus proved.
\end{proof}


\subsection{Unbounded context RHA with call-by-reference only mechanism}

\input{fif_ref-app}
Consider the example in Figure \ref{fig:ref-no-cnt-app}. 

Consider the run  $\rho = (\sseq{\varepsilon},en_1,0) \stackrel{0.1}{\rightarrow} 
  (\sseq{\varepsilon},(a_1,en_2),0.1) \stackrel{0}{\rightarrow} 
  (\sseq{a_1},en_2,0.1) \stackrel{0.1}{\rightarrow}$\\ 
  $(\sseq{a_1},(a_2,en_1),0.2) \stackrel{0}{\rightarrow} 
  (\sseq{a_1a_2},en_1,0.2) \stackrel{0.1}{\rightarrow} 
  (\sseq{a_1a_2},(a_1,en_2),0.3) \stackrel{0}{\rightarrow} 
  (\sseq{a_1a_2a_1},en_2,0.3) \stackrel{0.1}{\rightarrow} 
  (\sseq{a_1a_2a_1},(a_2,en_1),0.4) \stackrel{0}{\rightarrow} 
  (\sseq{a_1a_2a_1a_2},en_1,0.4) \stackrel{0.1}{\rightarrow} 
  (\sseq{a_1a_2a_1a_2},(a_1,en_2),0.5) \stackrel{0}{\rightarrow}$\\ 
  $(\sseq{a_1a_2a_1a_2a_1},en_2,0.5) \stackrel{0.5}{\rightarrow}
  (\sseq{a_1a_2a_1a_2a_1},ex_2,1) \stackrel{0}{\rightarrow} 
  (\sseq{a_1a_2a_1a_2},(a_1,ex_2),1) \stackrel{0}{\rightarrow}$\\ 
  $(\sseq{a_1a_2a_1a_2},ex_1,1) \stackrel{0}{\rightarrow} 
  (\sseq{a_1a_2a_1},(a_2,ex_1),1) \stackrel{0}{\rightarrow} 
  (\sseq{a_1a_2a_1},ex_2,1) \stackrel{0}{\rightarrow} 
  (\sseq{a_1a_2},(a_1,ex_2),1) \stackrel{0}{\rightarrow} 
  (\sseq{a_1a_2},ex_1,1) \stackrel{0}{\rightarrow} 
  (\sseq{a_1},(a_2,ex_1),1) \stackrel{0}{\rightarrow} 
  (\sseq{a_1},ex_2,1) \stackrel{0}{\rightarrow}  
  (\sseq{\varepsilon},(a_1,ex_2),1) \stackrel{0}{\rightarrow} 
  (\sseq{\varepsilon},ex_1,1)$. $\duration{\rho} = 1$. 
  
  Now consider another run 
  $\rho' = (\sseq{\varepsilon},en_1,0) \stackrel{0.1}{\rightarrow} 
  (\sseq{\varepsilon},(a_1,en_2),0.1) \stackrel{0}{\rightarrow} 
  (\sseq{a_1},en_2,0.1) \stackrel{0.9}{\rightarrow} 
  (\sseq{a_1},ex_2,1) \stackrel{0}{\rightarrow}
  (\sseq{\varepsilon},(a_1,en_2),1) \stackrel{0}{\rightarrow}
  (\sseq{\varepsilon},ex_1,1)$. 
  
  Note that the start and end configurations of both the runs are the same and $\duration{\rho'} = 1$. However, we can not apply context-sensitive contraction in this case. There can be several other runs like $\rho$ which can have unbounded contexts but have the same effect as $\rho'$. To be able to obtain $\rho'$ from $\rho$, we would need to apply contraction to the contexts too and shorten them in a sensible manner.  






==> dec-rha-ref.tex <==
% \subsection{Hybrid automata : Time bounded reachability \cite{BG13}}
% \todo{M: TODO : need to replace location with vertex for RHA explanation below.}
We mainly discuss the result (2) of Theorem \ref{thm:dec} here; 
the proof of (1) relies on the construction of a region abstraction for RHAs. 
Details can be found in Appendices \ref{dec}, \ref{contract}.   
Time bounded reachability was shown to be decidable for hybrid automata
with no negative rates and no diagonal constraints \cite{BG13}. 
The main idea here is that if there is a run $\rho$ between two configurations $(q_1,\nu_1)$ 
and $(q_2,\nu_2)$ in a hybrid automata $H$ such that 
$\duration{\rho} \leq T$ (called $T-$time bounded run), then there exists a {\it contracted} run $\rho'$
between the same configurations, such that $\duration{\rho'} \leq T$, length of $\rho'$ is atmost $C$, a constant
 exponential in $H$ and linear in $T$, and  is dependent on $rmax$ (maximal rate in $H$) and $cmax$ (largest constant in the constraints of $H$). The construction of $\rho'$ from $\rho$ relies on a {\it contraction} operator. 
 This operator identifies positions $i<j$ in $\rho$, such that all locations between $i$ and $j$ are visited before $i$ in $\rho$ and locations $l_i = l_j$ and $e_{i+1}=e_{j+1}$ the outgoing edges from $l_i$ and $l_j$ respectively. The operator then deletes all the locations $i+1, \dots, j$ and adds their time to the other occurrences before $i$. It then connects $l_i \stackrel{e_{j+1}}{\rightarrow}{l_{j+1}}$ with sum of time delays accompanying $e_{i+1}$ and $e_{j+1}$. 
This operator is used as many times as required until a fixpoint is reached.
  Care should be taken to ensure that the \textit{contracted run} is a valid run :  
it should satisfy the constraints. To ensure this, the run $\rho$ is first carefully partitioned into exponentially many pieces, 
so that contracting the pieces and concatenating them yields a valid run.

%We shall now describe briefly, how the contraction is carefully applied to partitions of $\rho$.
%so as to respect the constraints and yield a valid run. We know that $\duration{\rho} \leq T$. 
Firstly, to help track whether the valuations resulting from contraction satisfy constraints, 
the region information is stored in the locations to form another hybrid automaton $R(H)$.
Given $cmax$, the set of regions is $\{(a-1,a), [a,a] | a \in \{1, \cdots cmax\}\} \cup \{\mathbf{0^=},\mathbf{0^+},(cmax,+\infty)\}$. It differs from the classical region notion due to lack of fractional part ordering (no diagonal constraints) and special treatment of valuations which are 0. 
$R(H)$ checks whether a variable $x$ never changes from 0 before the next transition, or if it becomes $> 0$ before the next transition. This helps bound the number of sub-runs that are constructed later, and prevents the contraction operator from merging locations 
where x remains 0 with those where x becomes $>0$. The construction ensures that $H$ admits a run between two states  of duration T iff $R(H)$ admits a run between the same
states and for the same time $T$.

As the rest of the automaton is untouched, the equivalent of run $\rho$ in $R(H)$ is a run
same as $\rho$, but having region information along with locations. Let us continue to call the run in $R(H)$ as $\rho$. 
$\rho$ is called a \textit{type-0 run}. $\rho$ is chopped into fragments of duration  $\leq \frac{1}{rmax}$,
 each of which is called a \textit{type-1} run.  There will be atmost $T . rmax +1$ type-1 runs. 
Additionally, as $rmax$ is the maximal rate of growth of any variable, a variable changes its region atmost 
3 times such that, when starting in $(b,b+1)$ region, growing through $[b+1,b+1], (b+1,b+2)$, gets reset and stays in $[0,1)$. 
Each type-1 run is further split into type-2 runs based on region changes which is atmost 
3 times per variable. 
Thus each type-1 run is split into atmost $3. |\variables|$ type-2 runs. 
Respecting region changes ensures that constraints continue to be satisfied post contraction. 
Type-2 runs are again split into type-3 runs based on the first and last reset of a variable. 
This is to enable concatenation of consecutive contracted fragments by ensuring the valuations in the start configuration and end configuration of each fragment are compatible with their 
neighbors. Each type-2 run is split into atmost $2 . |\variables| + 1$ type-3 runs. 
The contraction is applied to type-3 runs, removing second occurrences of loops. 
Hence, each contracted type-3 run will be atmost 
$|Loc'|^2+1$ long (Lemma 7 of \cite{BG13}), where $Loc'$ is the set of locations of $R(H)$. 
Note that $|Loc'| = |Loc| . (2.cmax+1)^{|\variables|}$ where $Loc$ is the set of locations of $H$.
After concatenating these contracted type-3 runs, we get contracted type-2 runs with the same start and end states.
These contracted type-2 runs are then concatenated to obtain a run $\rho'$ of 
that has the same start and end states as $\rho$, $\duration{\rho'} = \duration{\rho}$ 
and $|\rho'|\leq C = 24 . (T . rmax +1 ) . |\variables| ^2 . |Loc|^2 . (2 . cmax + 1)^{2 . |\variables|}$. To solve time-bounded reachability, we  nondeterministically guess a run of length at most $C$, and solve an  LP to check if there are time delays and valuations for each step to make the run feasible.
\begin{theorem}
 \label{thm:dec-ref}
 Time bounded reachability is decidable for bounded context RHA using only call-by-reference mechanism.
\end{theorem}
\begin{proof}
We adapt the contraction operator of \cite{BG13} and make it {\it context-sensitive}.  This operator
respects the context of the RHA configurations. We split a given run $\rho$ of the RHA into type-3 runs exactly as done for hybrid automata \cite{BG13}. While applying contraction, 
we identify the second occurence of a loop by matching not just the location, but by the (context, location) pair in the configurations. The context matching ensures that we do not alter the sequence of recursive calls made in the contracted run, thus maintaining validity w.r.t recursion. The second occurences of a (location,context) pair are then deleted and the time delays are added to their first occurence in the loop.  
We match the (context, location) pair as opposed to only locations in \cite{BG13}. Thus, the size of the contracted type-3 run is atmost $ (\alpha . |Q|. (2.cmax+1)^{|\variables|})^2 +1$, where 
 $Q=\bigcup_{i=1}^nQ_i$ is the union of the set of vertices $Q_i$ of all the $n$ components of the RHA, $|Q|.(2.cmax+1)^{|\variables|}$ is the number of vertices in the region RHA, $K$ is the context bound, and $\alpha=\sum\limits_{i=1}^K n^i$. There are atmost $\alpha$ different contexts of size atmost $K$ with any sequence of the $n$ boxes including a box being called more than once.  
Thus our contracted run $\rho'$ has the same duration as $\rho$ and is of length atmost 
$|\rho'|\leq C = 24(T.rmax +1 ).|\variables| ^2 .(\alpha|Q|)^2 (2.cmax + 1)^{2 . |\variables|}$. 
To prove that the contracted run $\rho'$ is valid, we need to ensure that (i) 
$\rho'$ satisfies all the constraints as $\rho$, and has the same start and end configuration, 
 and (ii) recursive calls, returns and contexts are valid in the given RHA. All the variables are always passed by reference and the contexts have no valuations. Thus the precautions (in carefully splitting from type-0 to type-3 runs) taken in \cite{BG13} for hybrid automata suffice to ensure constraints are satisfied. 
 The second condition is satisfied due to context-sensitive contraction where in, the context is also matched 
 in the loop detection. Due to this, a context in the contracted run will be a valid successor of the preceding context. 
 Lemmas \ref{lem:cnt-len-type3}, \ref{lem:cnt-len} and  \ref{lem:cnt-valid} and Theorem \ref{thm:dec-ref} in Appendix \ref{contract} establish the correctness and hence the decidability of RHA with bounded context using pass-by-reference. 
    % Let us assume that $\rho'$ has a pair of consecutive configurations which are invalid as the call port configuration $c_1$ is not succeeded 
 %by the appropriate entry node configuration $c_2$. This means that during contraction, $c_2$ was deleted. This can happen only if there was a configuration $c_2'$ occuring before $c_1$ which 
% matched $c_2$ and hence this was deleted. But as the earlier/given run is valid, 
 %there would also be $c_1'$ preceeding $c_2'$ which would match $c_1$. Thus even $c_1$ would have been deleted by contraction, contradicting our assumption that the contracted run has $c_1$ but no matching $c_2$.
 %\todo{M: \textcolor{red}{Please read this carefully. Am I making a mistake here?}}
%
% Similar proof by contradiction can be given for any pair of configurations invalid w.r.t recursion. Detailed proof in appendix.
\end{proof}
\vspace{-.15cm}
\input{fig_ref-no-cnt_new.tex}
We show that our adaptation of contraction does not work on RHAs with unbounded context, as  in figure \ref{fig:ref-no-cnt}.
We can not apply context-sensitive contraction as the context 
might grow unboundedly and matching pairs may not be found within a type-3 run. 
In figure \ref{fig:ref-no-cnt}, consider a run $\rho_1$ 
where $B_1$ calls $B_2$ and $B_2$ calls $B_1$ until $x=1$
in $B_2$, after which the context shrinks to the first instance of $B_1$. In another run $\rho_2$,
$B_1$ calls $B_2$ once,  $x$ grows to be $1$ and $B_2$ returns to $B_1$. The context size is very small while 
achieving the same effect - same start and end configurations and same duration. 
To be able to obtain $\rho_2$ from $\rho_1$, we would need to apply contraction to the contexts too and shorten them in a sensible manner.
 Our context-sensitive contraction studied earlier does not alter the contexts and hence does not readily extend to this class  of RHA. We conjecture this to be decidable with a double layered contraction - one altering the contexts and the other altering the valuations (as seen in \cite{BG13}). 
%\begin{figure}[t]
 % \centering
 %\vspace*{-0.4cm}
 % \makebox[2cm]{\input{fig_ref-no-cnt.tex}}
  %\vspace*{-0.4cm}
  %\caption{Unbounded stack RHA with call-by-reference only mechanism where context-sensitive contraction fails. }
  %\vspace*{-0.4cm}
 %\label{fig:ref-no-cnt}
%\end{figure}



==> fig_ref-no-cnt_new.tex <==
 \begin{wrapfigure}{r}{0.4\textwidth}
 \vspace{-2em}
\begin{center}
\scalebox{0.75}{
\begin{tikzpicture}[node distance=4cm] 
  
  \draw(0, -0.2) rectangle (3,1.5);
  \draw (2.7, 1.7) node {$B_1$};

  \node[loc](n1) at (0, 0.8) {$en_{1}$};  
  
  \node[boxloc](f1) at (1.7, 0.8) {$\begin{array}{c} a_1{:}B_2\\ \end{array}$};
  \node[port](f1n1) [left of=f1,node distance = 7mm] {}; 
  \node[port](f1x1) [right of=f1,node distance = 7mm] {};

  \node[loc](x1) at (3, 0.8) {$ex_{1}$};

   \draw[trans] (n1)-- (f1n1) node[midway,above]{$ x{<}1$};
   \draw[trans] (f1x1)--(x1) {};   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   \draw(3.7, -0.2) rectangle (6.7,1.5);
  \draw (6.4, 1.7) node {$B_2$};

  \node[loc](n2) at (3.7, 0.8) {$en_{2}$};  
  
  \node[boxloc](f2) at (5.4, 0.8) {$\begin{array}{c} a_2{:}B_1\\ \end{array}$};
  \node[port](f2n1) [left of=f2,node distance = 7mm] {}; 
  \node[port](f2x1) [right of=f2,node distance = 7mm] {};

  \node[loc](x2) at (6.7, 0.8) {$ex_{2}$};

   \draw[trans] (n2)-- (f2n1) node[midway,above]{$x{<}1$};
   \draw[trans] (f2x1)--(x2) {};   
   \draw[trans] (n2) -- (4.5, 0.3) -- (6.2,0.3)node [midway, below] {$x{=}1$} -- (x2);
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tikzpicture}}
\vspace*{-0.2cm}
\caption{Unbounded context RHA}
\end{center}
%  \vspace*{-0.1cm}
\vspace{-2em}
\label{fig:ref-no-cnt}
 \end{wrapfigure}

==> rha-2-short.tex <==
\subsection{Unrestricted RHA with 2 stopwatches}
\begin{figure}[t]
  \centering
  \input{./figs/fig-rha-2.tex}
  \caption{Unrestricted RHA with 2 stopwatch : Decrement $c$ is $\db$, Increment $c$ is $\hf$}
\label{fig_undec_2swG-main}
\end{figure}

We prove that the reachability and termination problems are undecidable for 2 stopwatch unrestricted RHA.  
In order to obtain the undecidability result, we 
use a reduction from the halting problem 
for two counter machines. 
Our reduction uses a RHA with stopwatches $x,y$.
On entry into a main component for increment/decrement/zero check, 
we always have  $x=\frac{1}{2^c3^d}$, $y=0$ or $x=0, y=\frac{1}{2^c3^d}$, where
$c,d$ are the current values of the counters. On entering the entry node $en$ of
a main component corresponding to an instruction $\ell_i$, 
we have the configuration $(\langle \epsilon \rangle, en, (\frac{1}{2^c3^d},0))$ or 
$(\langle \epsilon \rangle, en, (0,\frac{1}{2^c3^d}))$
of the two stopwatch RHA.   

We shall now present the component for simulation of a decrement instruction for
counter $c$. 
Figure \ref{fig_undec_2swG-main} gives the 
complete set of main components needed for increment/decrement
counter $c$ and for testing if counter $d$ is zero.  
In all the components, the ticking variables are written below respective
locations in grey bags. To avoid clutter,  
the variables passed by value are written below each box.
We explain the   component $DB$ in Figure \ref{fig_undec_2swG-main}
which decrements counter $c$, by doubling $\frac{1}{2^c3^d}$.  Assume that 
$x=\frac{1}{2^c3^d}$ and $y=0$ on entering $DB$. Lets denote by $x_{old}$ the value
$\frac{1}{2^c3^d}$.   
A non-deterministic amount of time $t$ is spent at the entry node $en$ of  
$DB$. This makes $x=x_{old}$ and $y=t$, at the call port 
of $B_1:C_{DB}$. 
Both $x,y$ are passed by value to $C_{DB}$. 
At the entry node of $C_{DB}$, the rates of $x,y$ are zero. At sometime, the call port of $B_2:M_1$ 
is reached with   $x=x_{old}$ and $y=t$. $M_1$ is called by passing $x$ by value. At the entry node of $M_1$, 
a time $1-x_{old}$ is spent, obtaining $x=1,y=t+1-x_{old}$. 
We return from the exit node of $M_1$ to the return port of $B_2:M_1$, with $x=x_{old}, y=1+t-x_{old}$.
The rates of $x,y$ are both zero here. After some time,  we are at the call port of $B_3:M_1$. 
Here again, $M_1$ is called by passing $x$ by value. Going through $M_1$ again gives us 
$x=1, y=2-2x_{old}+t$. At the return port of $B_3$, we thus have $x=x_{old}, y=2-2x_{old}+t$. Again since the rates of $x,y$ are both zero at the return port of $B_3$, to get to the exit node of $C_{DB}$, $y$ must be exactly equal to 2. That is, 
$2x_{old}=t$. In that case, when we get back to the return port of $B_1:C_{DB}$, we have 
$x=x_{old}, y=t$, with the guarantee that $t=2x_{old}$. The rates of $x,y$ are both zero here, so we 
 get to the exit node $ex$ 
of $DB$ resetting $x$. Thus, when we reach the exit node of $DB$, we have  $x=0, y=\frac{1}{2^{c-1}3^d}$. 


==> rha-3-short.tex <==

\subsection{Glitchfree RHA with 3 stopwatches}
The proof of this is a straightforward adaptation of the techniques used 
in the case of unrestricted RHA with 2 stopwatches. 
The main difference here is that, at all times, we have to pass all variables either by value, or by reference. 
In fact, in our proof, we always pass {\it only by value}; thus, the result also holds for 
RHA where always variables are passed only by value.
This necessitates the need for an extra variable.

We use 3 stopwatches $x,y$ and $z$. 
 On entry into a main component for increment, decrement or zero check, 
we have as invariant $x=\frac{1}{2^c3^d}$, $y=z=0$
% or $x=0, y=\frac{1}{2^c3^d}$,
 where $c,d$ are the current values of the counters. 
On entering the entry node $en$ of a main component corresponding to an instruction $\ell_i$,
we have the configuration $(\langle \epsilon \rangle, en, (\frac{1}{2^c3^d},0,0))$ 
%or $(\langle \epsilon \rangle, en, (0,\frac{1}{2^c3^d}))$
of the three stopwatch RHA.  
In all the components, the ticking variables are written below respective locations, in grey bags. 
The tuple of variables written below each box denotes 
variables passed by value.
We present the  component for decrementing counter $c$. 

 Figure \ref{undec3main} gives the complete set of components
 needed for increment/decrement counter $c$ as well as  testing 
 if $c=0$. 
  We discuss the component 
    $DB$ 
which decrements counter $c$, by doubling $\frac{1}{2^c3^d}$.  Assume that 
$x=\frac{1}{2^c3^d}$ and $y=z=0$ on entering $DB$. Lets denote by $x_{old}$ the value
$\frac{1}{2^c3^d}$.   
A time $1-x_{old}$ is spent at the entry node $en_1$ of $DB$, resulting 
in $x=0, y=1-x_{old},z=0$ at location $l$. 
A non-deterministic amount of time $t$ is spent at $l$. 
This makes $x=t$ and $y=1-x_{old},z=0$, at the call port 
of $A_1:C_{DB}$. 
All variables $x,y,z$ are passed by value to $C_{DB}$. 

\begin{figure}[t]
  \centering
  \input{./figs/fig-rha-3.tex}
  \caption{Glitch-free RHA with 3 stopwatches : Decrement $c$ is $\db$, Increment $c$ is $\hf$.}
 \label{undec3main}
\end{figure}



At the entry node $en_2$ of $C_{DB}$, the rates of $y,z$ are one.
A time $x_{old}$ is spent at $en_2$, 
 obtaining $y=0,x=t$ and $z=x_{old}$  
  at $l_1$. 
  At $l_1$, a time $1-x_{old}$ is spent, obtaining 
  $x=1+t-x_{old}, y=1-x_{old}$ and $z=0$ at $l_2$.
  A time $x_{old}$ is spent at $l_2$ obtaining $x=1+t-x_{old}$, $y=0,z=x_{old}$ at $l_3$.
  A time $1-x_{old}$ is spent at $l_3$, obtaining $z=1,x=2+t-2x_{old}$ and $y=1-x_{old}$.
  To move out of $l_3$, $x$ must be 2; that is  
  possible iff 
   $t=2x_{old}$.
  In this case, from the return port of $A_1:C_{DB}$ (rates are all 0 here), we 
  reach the exit node $ex$ of $DB$ resetting $y$, obtaining $x=t=2x_{old},y=z=0$, thereby successfully 
  decrementing $c$. 


==> tb-rha-14-short.tex <==
\subsection{Glitchfree RHAs with 14 stopwatches}
We prove that  the problem of reaching a chosen vertex in an RHA  
within 18 units of total elapsed time is undecidable. 
In order to get the undecidability result, we use a reduction from the halting problem 
for two counter machines. Our reduction uses an RHA with atleast 14 stopwatches.
In our proof, we always pass variables {\it only by value}; thus, the result also holds for 
RHA where always variables are passed only by value.

We maintain 3 sets of stopwatches. The first set $X=\set{x_1,\cdots x_5}$ encodes correctly the current value of counter $c$;
the second set $Y=\set{y_1,\cdots y_5}$ encodes correctly the current value of counter $d$;
and third set $Z=\set{z_1,z_2,z_3}$ encodes the end of the $k$-th instruction.
An extra stopwatch $b$ is used to enforce urgency in some locations.
$b$ is zero at the entry nodes of all the main components.
Let $\variables$ denote the set of all 14 stopwatches.  
As an invariant of our reduction, 
on entry into a main component 
simulating the $(k+1)$th instruction, 
we have the values of $z_1,z_2,z_3$ as $1-\frac{1}{2^k}$,
the values of $x_1, \dots, x_5$ as 
$1-\frac{1}{2^{c+k}}$, and the values of $y_1, \dots, y_5$ as
$1-\frac{1}{2^{d+k}}$, where $c,d$ are the current values of 
the counters after simulating the first $k$ instructions. 
We will denote this by saying that at the beginning of the $k+1$th instruction, 
we have $\nu(Z)=1-\frac{1}{2^k}$, $\nu(X)=1-\frac{1}{2^{c+k}}$ and 
$\nu(Y)=1-\frac{1}{2^{d+k}}$. 

\begin{figure}[t]

\input{./figs/fig-tb-rha-14.tex}
 \caption{Time bounded reachability in 14 stopwatch RHA: Increment $c$. Note
   that the variables which tick in a location are indicated below it. $b$ ticks
   everywhere except in locations where it is specified as $\neg b$. Also
   $\varbar{S}$ denoted stopwatches $\variables - S$.  
 }
 \label{14main}
\end{figure}


We now present the increment instruction for counter $c$. 
 Assume that this is the $(k+1)$th instruction.  Figure \ref{14main} gives the figure 
for incrementing counter $c$.  At the entry node $en_1$ of 
the component $Inc~c$, we have $\nu(X)=1-\frac{1}{2^{c+k}}$, $\nu(Y)=1-\frac{1}{2^{d+k}}$ and $\nu(Z)=
1-\frac{1}{2^k}$, and $\nu(b)=0$.
The component $Inc~c$ has three subcomponents sequentially lined up one after the other: 
Let $\beta=\frac{1}{2^k}, \beta_c=\frac{1}{2^{c+k}}$, and $\beta_d=\frac{1}{2^{d+k}}$. 
The functionality of $Up_n^A$ for $A \in \{X,Y,Z\}$ and $n \in \{2,4\}$ is similar to the functionality of 
the subcomponents $Up_n^a$ and $Up_n^Z$ dealt in the proof of RTA with 5 clocks. 
 The entire construction and 
explanations can be found in the Appendix.



==> tb-rta-5-short.tex <==

\subsection{Unrestricted RTA with $5$ clocks under bounded time}
We prove that  the problem of reaching a chosen vertex in an RTA with 5 clocks,   
within 18 units of total elapsed time is undecidable. 
The main challenge here is that, apart from simulating the counter machine properly, we 
need to ensure that the total time elapsed is $<18$ units. 
We maintain 3 sets of clocks. The first set $X=\{x\}$ 
 encodes correctly the current value of counter $c$;
the second set $Y=\{y\}$  
encodes correctly the current value of counter $d$;
the third set $Z=\{z_1,z_2\}$ of 2 clocks 
helps in zero-check.  
An extra clock $b$ is used to enforce urgency in some locations.
Let $\mathcal{X}$ denote the set of all 5 clocks.  
On entry into a main component 
simulating the $(k+1)$th instruction, 
we have the values of $z_1,z_2$ as $1-\frac{1}{2^k}$,
the value of $x$ as 
$1-\frac{1}{2^{c+k}}$, the value of $y$ as
$1-\frac{1}{2^{d+k}}$, and $b=0$, where $c,d$ are the current values of 
the counters after simulating the first $k$ instructions. 
 If the $(k+1)$th instruction $\ell_{k+1}$ is an 
increment counter $c$ instruction, then after the simulation 
of $\ell_{k+1}$, we need $z_1=z_2=1-\frac{1}{2^{k+1}}$,
$\nu(x)=1-\frac{1}{2^{c+k+2}}$ and 
$\nu(y)=1-\frac{1}{2^{d+k+1}}$. We show by our construction that, 
 the time taken to simulate the $(k+1)$th instruction is 
 $<\frac{9}{2^k}$. Thus, the time taken to simulate the first 
 instruction is $<9$, the second instruction is $<\frac{9}{2} \dots$, so that the total time taken in simulating 
 the two counter machine is $<18$.
 
  Figure \ref{5clk} gives the complete set of components for incrementing counter $c$. 
 Assume that this is the $(k+1)$th instruction. The tuple of clocks written below each box denotes 
clocks passed by value.
     At the entry node $en_1$ of 
the component $Inc~c$, we have $\nu(x)=1-\frac{1}{2^{c+k}}$, $\nu(y)=1-\frac{1}{2^{d+k}}$ and $\nu(Z)=
1-\frac{1}{2^k}$, and $\nu(b)=0$.

\begin{figure}[t]

\input{./figs/fig-tb-rta-5.tex}
 \caption{Unrestricted RTA with 5 clocks: Increment $c$. Note that $\varbar{S} = \variables-S$ and $a \in \set{x,y}$. 
 $C_{z_2}^{z_1=}$ is obtained by instantiating $a=z_1$ in  $C_{z_2}^{a=}$.  
 The component $\chkAn{a}{4}$ is similar to $\chkAn{a}{2}$. It has 4 calls to $\DEq{a}$ inside it each time passing only $z_2$ by reference.}
 \label{5clk}
\end{figure}





The component $Inc~c$ has three subcomponents sequentially lined up one after the other: 
Let $\beta=\frac{1}{2^k}, \beta_c=\frac{1}{2^{c+k}}$, and $\beta_d=\frac{1}{2^{d+k}}$.
\begin{enumerate}
\item The first subcomponent 
is $Up_2^y$.  
If $Up_2^y$ is entered with $\nu(y)=1-\beta_d$, then on exit, 
we have $\nu(y)=1-\frac{\beta_d}{2}$. The values of $X,Z$ are unchanged. Also, the total time elapsed 
in $Up_2^y$ is $\leq \frac{5\beta}{2}$.
\item The next subcomponent is $Up_4^x$.  
If $Up_4^x$ is entered with $\nu(x)=1-\beta_c$, then on exit, 
we have $\nu(x)=1-\frac{\beta_c}{4}$. The values of $Z,Y$ are unchanged. Also, the total time elapsed 
in $Up_4^x$ is $\leq \frac{11\beta}{4}$.
\item The next subcomponent is $Up_2^Z$ updates the value of $Z$. 
If $Up_2^Z$ is entered with $\nu(Z)=1-\beta$, then on exit, 
we have $\nu(Z)=1-\frac{\beta}{2}$. The values of $X,Y$ are unchanged. Also, the total time elapsed 
in $Up_2^Z$ is $\leq \frac{5\beta}{2}$. 
\item Thus, at the end of the $Inc~c$, we obtain $\nu(Z)=1-\frac{1}{2^{k+1}}$, 
$\nu(x)= 1-\frac{1}{2^{c+k+2}}$, $\nu(y)=1-\frac{1}{2^{d+k+1}}$. Also, the total time elapsed 
in $Inc~c$ is $\leq [\frac{5}{2}+\frac{11}{4}+\frac{5}{2}]\beta < 8 \beta$.
\end{enumerate}
The Appendix has a detailed explanation about the component $Up_2^y$, and the total time elapsed.
We quickly explain the differences in a decrement $c$ component, and zerocheck component.
\begin{itemize}
\item The main component $Dec~c$ will have the subcomponents 
   $Up_2^y$ and  $Up_2^Z$ lined up sequentially. The functionality 
   $Up_2^Z$ and  $Up_2^y$ are the same as the one in $Inc~c$.
  The total time spent in $Dec~c$ is also, less than $8 \beta$. 
\item The main component $ZeroCheck$ will have the subcomponents 
   $Up_2^y$ and $Up_2^x$ and $Up_2^Z$ lined up sequentially. The functionality 
   $Up_2^Z,Up_2^x$ and  $Up_2^y$ are the same as the one in $Inc~c$. 
   After these three, we invoke the subcomponent $ZC$.
   $ZC$ is called by passing all clocks by value. 
         At the entry node $en$ of 
   $ZC$, we have two transitions, one on $z_1=1 \wedge x=1$ leading to an exit node $ex$, and another 
   one on $z_1= 1\wedge x \neq 1$ leading to $ex'$. 
   Since $z_1=\frac{1}{2^k}$, 
        a time elapse $\frac{\beta}{2}=\frac{1}{2^{k+1}}$ makes $z_1=1$. 
        If the same elapse also makes $x=1$, 
          then 
   we know that $x$ on entry was $1-\frac{1}{2^{c+k+1}}= 1-\frac{1}{2^{k+1}}$ 
   impying that $c=0$. 
   Likewise, if $z_1$ attains 1, but $x$ does not, then $c \neq 0$.  
 Since all clocks are passed by value, at the return port of $ZC$ within the main component
 $ZeroCheck$, we regain back the clock values obtained 
 after going through $Up_2^Z,Up_2^x$ and  $Up_2^y$: that is, 
 $\nu(Z)=1-\frac{\beta}{2}$, $\nu(x)=1-\frac{\beta_c}{2}$ and $\nu(y)=1-\frac{\beta_d}{2}$. 
  The time elapsed in $ZC$ is $\frac{\beta}{2}$. The times elapsed in   
     $Up_2^Z$ and $Up_2^x$ and $Up_2^y$ are same as calculated 
     in the case of Increment $c$. Thus, the total time elapsed here is $< 8\beta+\beta=9\beta$.
 \end{itemize}

